Vanishing, Unbounded and Angular Shifts on the Quotient of the Difference and the Derivative of a Meromorphic Function

We show that for a vanishing period difference operator of a meromorphic function \( f \), there exist the following estimates regarding proximity functions, \[ \lim_{\eta \to 0} m_\eta\left(r, \frac{\Delta_\eta f - a\eta}{f' - a} \right) = 0 \] and \[ \lim_{r \to \infty} m_\eta\left(r, \frac{\Delta_\eta f - a\eta}{f' - a} \right) = 0, \] where \( \Delta_\eta f = f(z + \eta) - f(z) \), and \( |\eta| \) is less than an arbitrarily small quantity \( \alpha(r) \) in the second limit. Then, under certain assumptions on the growth, restrictions on the period tending to infinity, and on the value distribution of a meromorphic function \( f(z) \), we have \[ m\left(r, \frac{\Delta_\omega f - a\omega}{f' - a} \right) = S(r, f'), \] as \( r \to \infty \), outside an exceptional set of finite logarithmic measure. Additionally, we provide an estimate for the angular shift under certain conditions on the shift and the growth. That is, the following Nevanlinna proximity function satisfies \[ m\left(r, \frac{f(e^{i\omega(r)}z) - f(z)}{f'} \right) = S(r, f), \] outside an exceptional set of finite logarithmic measure. Furthermore, the above estimates yield additional applications, including deficiency relations between \( \Delta_\eta f \) (or \( \Delta_\omega f \)) and \( f' \), as well as connections between \( \eta/\omega \)-separated pair indices and \( \delta(0, f') \).

==> oscillation.tex <==
\section{The oscillation of the difference with angle}

For a meromorphic function $f$, we put
$$
v(r,f,\theta)=\int_{0}^{2\pi}\left(\sup_{t\in[\tau,\tau+\theta]}\log\left|f(re^{it})\right|-\log\left|f(re^{i\tau})\right|\right)\frac{{\rm d}\tau}{2\pi},
$$
$$
\lambda(r)=\min\left\{1,\left(\log^+\frac{T(r)}{\log r}\right)^{-1}\right\}.
$$

\begin{proposition}
    \label{op1}
    Let $f$ be a transcendental meromorphic function in the complex plane. Let $\varepsilon>0$. Then we have
    $$v(r,f,\lambda(r)^{20})\le\varepsilon T(r)$$
    for all $r>e$ outside a set of logarithmic density zero.
\end{proposition}

To prove this proposition, we begin with the following lemma:

\begin{lemma}
    \label{ol1}
    Let $f$ be a transcendental meromorphic function in the complex plane. Let $1<\sigma<e$. Then we have
    $$
    \int_r^{\sigma r}\frac{v(t,f,(\log\sigma)^{10})}{t}{\rm d}t<508(\log\sigma)^2(T(\sigma^3r,f)+c)
    $$
\end{lemma}

\iffalse
Here, we can divide the integral interval into $[0, \pi-\frac{1}{2}\omega(r)]$, $(\pi-\frac{1}{2}\omega(r), 2\pi-\omega(r)]$, and $(2\pi-\omega(r),2\pi)$. Exactly, we can write $$\int_0^{2\pi}\sup_{\eta<\omega(r)}\frac{1}{|re^{i\theta+i\eta}-a_k|^\delta}\frac{{\rm d}\theta}{2\pi}=\int_0^{\pi-\frac{1}{2}\omega(r)}\frac{1}{|re^{i\theta}-a_k|^\delta}\frac{{\rm d}\theta}{2\pi}+\int_{\pi-\frac{1}{2}\omega(r)}^{2\pi-\omega(r)}\frac{1}{|re^{i\theta+i\omega(r)}-a_k|^\delta}\frac{{\rm d}\theta}{2\pi}+\int_{2\pi-\omega(r)}^{2\pi}\frac{1}{|r-a_k|^\delta}\frac{{\rm d}\theta}{2\pi}.$$
\fi
